Exponential decay of the resonance error in numerical homogenization via parabolic and elliptic cell problems

This paper presents two new approaches for finding the homogenized coefficients of multiscale elliptic PDEs. Standard approaches for computing the homogenized coefficients suffer from the so-called resonance error, originating from a mismatch between the true and the computational boundary conditions. Our new methods, based on solutions of parabolic and elliptic cell-problems, result in an exponential decay of the resonance error.

==> img/ModEllApproach_q1q4.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44706,0.74118}%
\definecolor{mycolor2}{rgb}{0.85098,0.32549,0.09804}%
%
\begin{tikzpicture}

\begin{axis}[%
width=7.734in,
height=8.04in,
at={(1.297in,1.085in)},
scale only axis,
xmode=log,
xmin=1,
xmax=20,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$R$},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\|a^{0}_{T,R,L,N}  - a^{0}\|_{F}$},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.237,0.333)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0.440536317049787\\
1.03072240652209	0.450004534224021\\
1.06238867930668	0.452530862587029\\
1.09502781619681	0.449667702942637\\
1.128669705919	0.442762788987875\\
1.1633451554534	0.432906964984152\\
1.19908591824474	0.420701088988648\\
1.23592472327997	0.406656920841575\\
1.27389530505928	0.390986665714106\\
1.31303243448788	0.373890931389088\\
1.35337195071691	0.355402398986571\\
1.39495079396242	0.335659260799249\\
1.43780703933284	0.314684625939258\\
1.48197993169554	0.292513517174122\\
1.52750992161467	0.26924497252042\\
1.57443870239304	0.244995926970895\\
1.62280924825206	0.219976852127389\\
1.67266585368467	0.19423971709282\\
1.72405417401718	0.167956355554472\\
1.77702126721744	0.141393779568453\\
1.83161563698728	0.114601756701932\\
1.88788727717902	0.0879042328762961\\
1.94588771757639	0.0614156357072889\\
2.00567007108211	0.0354595423859881\\
2.06728908235507	0.0102361627686689\\
2.13080117794186	0.0139470441183656\\
2.19626451794833	0.0367838802510472\\
2.26373904929878	0.0579372542957475\\
2.33328656063125	0.0769921255721296\\
2.40497073887949	0.0934920889099582\\
2.47885722759307	0.106845409641916\\
2.5550136870494	0.116279853719805\\
2.63350985621243	0.120776029473353\\
2.71441761659491	0.119038887390665\\
2.79781105808265	0.109722026708325\\
2.88376654678106	0.0927534531322725\\
2.97236279494606	0.0722036291143319\\
3.06368093306352	0.0554849745314575\\
3.15780458414306	0.0434538130646888\\
3.25481994029442	0.0329538230350217\\
3.35481584165634	0.0227211345684462\\
3.45788385775044	0.0126141630842952\\
3.56411837133441	0.00293986481143105\\
3.67361666483139	0.00589049532568409\\
3.78647900941465	0.0134321132149595\\
3.90280875682923	0.0192453264163819\\
4.0227124340345	0.0229473565094008\\
4.14629984075437	0.0242776693697061\\
4.27368415002449	0.0231699708551524\\
4.40498201182854	0.0198964242143794\\
4.54031365991841	0.0152135448735822\\
4.67980302191621	0.0107490285447129\\
4.82357783279881	0.0089853684275838\\
4.97176975186899	0.0100140596806243\\
5.12451448332012	0.00671095761299412\\
5.281951900505	0.000495029977069905\\
5.44422617402243	0.00631937380769909\\
5.61148590373893	0.0115222948896911\\
5.78388425486656	0.0149814777579181\\
5.96157909822127	0.0164501313379987\\
6.1447331547904	0.0159743296269999\\
6.33351414474162	0.0137628487315525\\
6.52809494100976	0.0100798705530983\\
6.72865372760224	0.00446567822876831\\
6.93537416276799	0.00412530365542707\\
7.14844554717933	0.0105806375808964\\
7.36806299728077	0.0123909934765335\\
7.59442762396358	0.0112901396316537\\
7.82774671672956	0.00776172877231696\\
8.06823393351286	0.00260550457549991\\
8.31610949633354	0.0029837149850036\\
8.57160039296208	0.00748040245339621\\
8.83494058477954	0.00868534638581675\\
9.10637122102363	0.00637911114484424\\
9.38614085961695	0.00373484518716738\\
9.67450569477967	0.000252827976362169\\
9.97172979163494	0.00297453254078794\\
10.278085328022	0.00465797990404615\\
10.5938528437381	0.00424249652362918\\
10.9193214974386	0.00270757999640547\\
11.2547893314283	7.04282403402035e-05\\
11.6005635445889	0.00286529906989019\\
11.9569607736911	0.00412477095521535\\
12.324307383349	0.00322829022397708\\
12.7029397648835	0.000670296116673463\\
};
\addlegendentry{$q=1$}

\addplot [color=mycolor1, dashed]
  table[row sep=crcr]{%
1	1\\
1.03072240652209	0.941275090254729\\
1.06238867930668	0.885998795534048\\
1.09502781619681	0.833968596231893\\
1.128669705919	0.784993865687785\\
1.1633451554534	0.738895171774678\\
1.19908591824474	0.695503619500994\\
1.23592472327997	0.654660232218289\\
1.27389530505928	0.616215369167452\\
1.31303243448788	0.580028177229444\\
1.35337195071691	0.545966074871931\\
1.39495079396242	0.513904266401097\\
1.43780703933284	0.483725284738983\\
1.48197993169554	0.455318561051181\\
1.52750992161467	0.428580019648104\\
1.57443870239304	0.403411696675643\\
1.62280924825206	0.379721381198179\\
1.67266585368467	0.357422277358966\\
1.72405417401718	0.336432686380112\\
1.77702126721744	0.316675707237081\\
1.83161563698728	0.298078954911063\\
1.88788727717902	0.280574295186946\\
1.94588771757639	0.26409759502525\\
2.00567007108211	0.248588487593449\\
2.06728908235507	0.233990151095811\\
2.13080117794186	0.220249100591427\\
2.19626451794833	0.207314992037718\\
2.26373904929878	0.195140437841462\\
2.33328656063125	0.183680833241569\\
2.40497073887949	0.172894192887522\\
2.47885722759307	0.162740997014721\\
2.5550136870494	0.153184046653176\\
2.63350985621243	0.144188327339053\\
2.71441761659491	0.135720880829745\\
2.79781105808265	0.12775068435247\\
2.88376654678106	0.120248536943974\\
2.97236279494606	0.113186952464939\\
3.06368093306352	0.106540058897093\\
3.15780458414306	0.100283503554105\\
3.25481994029442	0.0943943638589509\\
3.35481584165634	0.0888510633608718\\
3.45788385775044	0.0836332926842332\\
3.56411837133441	0.0787219351196518\\
3.67361666483139	0.0740989965847772\\
3.78647900941465	0.069747539698121\\
3.90280875682923	0.0656516217243941\\
4.0227124340345	0.0617962361639984\\
4.14629984075437	0.0581672577726702\\
4.27368415002449	0.0547513908098402\\
4.40498201182854	0.0515361203261043\\
4.54031365991841	0.0485096663113324\\
4.67980302191621	0.0456609405354262\\
4.82357783279881	0.0429795059235992\\
4.97176975186899	0.0404555383173395\\
5.12451448332012	0.0380797904809574\\
5.281951900505	0.0358435582218443\\
5.44422617402243	0.0337386485003171\\
5.61148590373893	0.0317573494122086\\
5.78388425486656	0.0298924019342276\\
5.96157909822127	0.0281369733285708\\
6.1447331547904	0.0264846321093453\\
6.33351414474162	0.0249293244790873\\
6.52809494100976	0.0234653521490424\\
6.72865372760224	0.0220873514619488\\
6.93537416276799	0.0207902737408338\\
7.14844554717933	0.0195693667918239\\
7.36806299728077	0.0184201574932019\\
7.59442762396358	0.01733843540692\\
7.82774671672956	0.0163202373525244\\
8.06823393351286	0.015361832886976\\
8.31610949633354	0.0144597106371664\\
8.57160039296208	0.0136105654350561\\
8.83494058477954	0.0128112862083003\\
9.10637122102363	0.012058944581997\\
9.38614085961695	0.011350784149796\\
9.67450569477967	0.0106842103750612\\
9.97172979163494	0.0100567810850862\\
10.278085328022	0.00946619752353662\\
10.5938528437381	0.00891029592833602\\
10.9193214974386	0.00838703960414083\\
11.2547893314283	0.00789451146035765\\
11.6005635445889	0.00743090698736514\\
11.9569607736911	0.00699452764520662\\
12.324307383349	0.00658377464053106\\
12.7029397648835	0.00619714306898267\\
};
\addlegendentry{$O(R^{-3})$}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0.620694889087441\\
1.03072240652209	0.638178810133231\\
1.06238867930668	0.649156430536789\\
1.09502781619681	0.655138547910528\\
1.128669705919	0.657489431515096\\
1.1633451554534	0.657198604531521\\
1.19908591824474	0.654895545695219\\
1.23592472327997	0.650953719351936\\
1.27389530505928	0.645583816704899\\
1.31303243448788	0.638900249170771\\
1.35337195071691	0.630959938866106\\
1.39495079396242	0.621786791229536\\
1.43780703933284	0.611384685879775\\
1.48197993169554	0.599749846553449\\
1.52750992161467	0.586882788450358\\
1.57443870239304	0.572795463421744\\
1.62280924825206	0.557507875226863\\
1.67266585368467	0.541042236587089\\
1.72405417401718	0.52342349220263\\
1.77702126721744	0.504682759097927\\
1.83161563698728	0.48486077305712\\
1.88788727717902	0.464011458592364\\
1.94588771757639	0.442205196413563\\
2.00567007108211	0.419532608535747\\
2.06728908235507	0.39610920746413\\
2.13080117794186	0.372081100093322\\
2.19626451794833	0.347632752793833\\
2.26373904929878	0.322996731967732\\
2.33328656063125	0.298466671739124\\
2.40497073887949	0.274413311615976\\
2.47885722759307	0.251302754539797\\
2.5550136870494	0.229710144064259\\
2.63350985621243	0.210307524853493\\
2.71441761659491	0.193772702570499\\
2.79781105808265	0.180487202039952\\
2.88376654678106	0.169777974871845\\
2.97236279494606	0.158896248829832\\
3.06368093306352	0.144772232205046\\
3.15780458414306	0.128317814670888\\
3.25481994029442	0.111568888249097\\
3.35481584165634	0.0953627951041226\\
3.45788385775044	0.0799963285534517\\
3.56411837133441	0.0656102812195364\\
3.67361666483139	0.0522912646913458\\
3.78647900941465	0.0400996823153349\\
3.90280875682923	0.0290800014217222\\
4.0227124340345	0.0192677818175013\\
4.14629984075437	0.0106996880743809\\
4.27368415002449	0.00343142391966278\\
4.40498201182854	0.00242918305181006\\
4.54031365991841	0.00666404222112327\\
4.67980302191621	0.00887095066839261\\
4.82357783279881	0.00856057745680039\\
4.97176975186899	0.00636562092408932\\
5.12451448332012	0.00500663231106635\\
5.281951900505	0.00427142865753483\\
5.44422617402243	0.00343382887402222\\
5.61148590373893	0.00252877285554654\\
5.78388425486656	0.00164022636551953\\
5.96157909822127	0.00097537580975704\\
6.1447331547904	0.000539309889174722\\
6.33351414474162	0.000335362909394732\\
6.52809494100976	0.000308072696186157\\
6.72865372760224	0.000102205961264173\\
6.93537416276799	0.000750904770192129\\
7.14844554717933	0.00102872716262414\\
7.36806299728077	0.000776233682938998\\
7.59442762396358	0.0004278159291492\\
7.82774671672956	7.38595160060251e-05\\
8.06823393351286	0.000241398931970171\\
8.31610949633354	0.000483582367165947\\
8.57160039296208	0.000595791074964436\\
8.83494058477954	0.000425075238928985\\
9.10637122102363	5.06953348923256e-05\\
9.38614085961695	7.14581376098922e-05\\
9.67450569477967	0.00012896397226525\\
9.97172979163494	0.000106031236807413\\
10.278085328022	2.99946970730991e-05\\
10.5938528437381	3.49936716044219e-05\\
10.9193214974386	1.53921794238121e-06\\
11.2547893314283	0.000141808557193479\\
11.6005635445889	0.000100537504453269\\
11.9569607736911	3.87577389137084e-05\\
12.324307383349	2.0384849620525e-06\\
12.7029397648835	2.30820327382641e-05\\
};
\addlegendentry{$q=4$}

\addplot [color=mycolor2, dashed]
  table[row sep=crcr]{%
1	0.999999999999999\\
1.03072240652209	0.859590118471982\\
1.06238867930668	0.738895171774678\\
1.09502781619681	0.635146988244172\\
1.128669705919	0.545966074871931\\
1.1633451554534	0.469307042980847\\
1.19908591824474	0.403411696675642\\
1.23592472327997	0.346768708138399\\
1.27389530505928	0.298078954911063\\
1.31303243448788	0.256225724166006\\
1.35337195071691	0.220249100591427\\
1.39495079396242	0.189323950470732\\
1.43780703933284	0.162740997014721\\
1.48197993169554	0.139890552904132\\
1.52750992161467	0.120248536943974\\
1.57443870239304	0.103364454117754\\
1.62280924825206	0.0888510633608718\\
1.67266585368467	0.0763754960807334\\
1.72405417401718	0.0656516217243941\\
1.77702126721744	0.0564334852959498\\
1.83161563698728	0.0485096663113324\\
1.88788727717902	0.0416984298115946\\
1.94588771757639	0.0358435582218443\\
2.00567007108211	0.0308107684583726\\
2.06728908235507	0.0264846321093453\\
2.13080117794186	0.0227659280525591\\
2.19626451794833	0.0195693667918239\\
2.26373904929878	0.0168216343190056\\
2.33328656063125	0.0144597106371664\\
2.40497073887949	0.0124294243796725\\
2.47885722759307	0.0106842103750612\\
2.5550136870494	0.00918404166207845\\
2.63350985621243	0.00789451146035765\\
2.71441761659491	0.00678604404148726\\
2.79781105808265	0.00583321640157813\\
2.88376654678106	0.00501417517770526\\
2.97236279494606	0.00431013543504294\\
3.06368093306352	0.00370494982923886\\
3.15780458414306	0.00318473826264818\\
3.25481994029442	0.00273756954049201\\
3.35481584165634	0.00235318772563682\\
3.45788385775044	0.00202277691586697\\
3.56411837133441	0.00173875904875248\\
3.67361666483139	0.00149462009671138\\
3.78647900941465	0.00128476066600274\\
3.90280875682923	0.00110436757309744\\
4.0227124340345	0.000949303452995446\\
4.14629984075437	0.000816011867626218\\
4.27368415002449	0.000701435737967366\\
4.40498201182854	0.000602947229099851\\
4.54031365991841	0.000518287480094295\\
4.67980302191621	0.000445514796416801\\
4.82357783279881	0.00038296011663294\\
4.97176975186899	0.000329188732026553\\
5.12451448332012	0.000282967381162347\\
5.281951900505	0.000243235964697048\\
5.44422617402243	0.000209083231710583\\
5.61148590373893	0.000179725879916605\\
5.78388425486656	0.000154490590409996\\
5.96157909822127	0.000132798584913335\\
6.1447331547904	0.000114152351338566\\
6.33351414474162	9.8124233210973e-05\\
6.52809494100976	8.43466212507928e-05\\
6.72865372760224	7.25035221536805e-05\\
6.93537416276799	6.23233111977183e-05\\
7.14844554717933	5.3572502456013e-05\\
7.36806299728077	4.60503937330048e-05\\
7.59442762396358	3.95844634046351e-05\\
7.82774671672956	3.40264135876401e-05\\
8.06823393351286	2.92487688869763e-05\\
8.31610949633354	2.51419527127156e-05\\
8.57160039296208	2.16117741109402e-05\\
8.83494058477954	1.85772674684128e-05\\
9.10637122102363	1.59688355440587e-05\\
9.38614085961695	1.37266532371771e-05\\
9.67450569477967	1.17992954823688e-05\\
9.97172979163494	1.01425578015754e-05\\
10.278085328022	8.71844246226513e-06\\
10.5938528437381	7.49428698902965e-06\\
10.9193214974386	6.44201504076304e-06\\
11.2547893314283	5.53749247208779e-06\\
11.6005635445889	4.75997381011967e-06\\
11.9569607736911	4.0916264513643e-06\\
12.324307383349	3.51712166607134e-06\\
12.7029397648835	3.02328302961864e-06\\
};
\addlegendentry{$O(R^{-5})$}

\end{axis}
\end{tikzpicture}%

==> img/tot_err_optTL_diffq_GloriaLeBris.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44706,0.74118}%
\definecolor{mycolor2}{rgb}{0.85098,0.32549,0.09804}%
%
\begin{tikzpicture}

\begin{axis}[%
width=.8\linewidth,
height=2.5in,
%at={(1.63in,1.171in)},
scale only axis,
xmode=log,
xmin=1,
xmax=15,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={$R$},
ymode=log,
ymin=0.0001,
ymax=10,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\|a^{0,R,T} - a^0 \|_F$},
axis background/.style={fill=white},
title style={font=\bfseries},
title={$k_o=2/3$, $k_T = \sqrt{50c/\lambda}$},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	3.11910210577215\\
1.05	3.22296156542475\\
1.1	3.33403003237762\\
1.15	3.42289144064882\\
1.2	3.46345470929223\\
1.25	3.44591508458213\\
1.3	3.37195359815166\\
1.35	3.24761200590638\\
1.4	3.07943572896535\\
1.45	2.86922733185742\\
1.5	2.62025512175085\\
1.55	2.34041669629489\\
1.6	2.04349374056334\\
1.65	1.7446764516432\\
1.7	1.45761353920941\\
1.75	1.18908631716467\\
1.8	0.944344958977297\\
1.85	0.724353148021206\\
1.9	0.529039462806468\\
1.95	0.356583190837845\\
2	0.20692366736688\\
2.1	0.0611414047278091\\
2.15	0.151210759892746\\
2.2	0.234400572232124\\
2.25	0.30585742166888\\
2.35	0.411754320790213\\
2.4	0.448089425944363\\
2.5	0.495167102617949\\
2.55	0.50889790070124\\
2.65	0.520340506073107\\
2.7	0.519273922985605\\
2.8	0.506251736136119\\
2.9	0.479051161639354\\
2.95	0.46055195101913\\
3.05	0.413182221259128\\
3.15	0.355067994679942\\
3.25	0.293018190188025\\
3.35	0.234361970461589\\
3.45	0.179586526731198\\
3.55	0.124324929878111\\
3.65	0.0669326847032808\\
3.75	0.00969652722138864\\
3.9	0.0764034655205422\\
4	0.13054177893757\\
4.1	0.181687459627751\\
4.25	0.248244061936462\\
4.35	0.279577182437926\\
4.5	0.285706050868325\\
4.65	0.228903963536993\\
4.75	0.173931403985175\\
4.9	0.0932021049596424\\
5.05	0.026670767343363\\
5.2	0.0233420041462699\\
5.4	0.0694564197984789\\
5.55	0.0983400168935017\\
5.7	0.107284672370006\\
5.9	0.110510270404784\\
6.05	0.107766709334476\\
6.25	0.0886984521496751\\
6.45	0.0610363105330081\\
6.65	0.0274109952784874\\
6.85	0.00813290896983116\\
7.05	0.044790212825315\\
7.25	0.081852176843293\\
7.45	0.102194689836042\\
7.7	0.0785192093846885\\
7.95	0.0267171435143002\\
8.15	0.00392122611755131\\
8.4	0.0266259492387496\\
8.65	0.0463800541780114\\
8.95	0.0514694175708476\\
9.2	0.0404167322592886\\
9.5	0.0227063579344532\\
9.75	0.00739867611457411\\
10.05	0.01999989246167\\
10.35	0.0459118252276218\\
10.7	0.0418568063741269\\
11	0.0132129931299929\\
11.35	0.0147163662685165\\
11.7	0.0234406808896295\\
12.05	0.0291608099002786\\
};
\addlegendentry{$q=1$}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	3.17055832626761\\
1.05	3.24151142897256\\
1.1	3.32035607912141\\
1.15	3.39420786243201\\
1.2	3.449298978104\\
1.25	3.4767857198654\\
1.3	3.47564178763346\\
1.35	3.45070739878821\\
1.4	3.40981024772714\\
1.45	3.35988652264341\\
1.5	3.30566149924306\\
1.55	3.24791640068688\\
1.6	3.18475764507571\\
1.65	3.1129159004764\\
1.7	3.03023615685993\\
1.75	2.93522246355593\\
1.8	2.82841837322378\\
1.85	2.7104546750357\\
1.9	2.58337711079917\\
1.95	2.44885356210162\\
2	2.30931008146995\\
2.1	2.02267056705055\\
2.15	1.87945729596353\\
2.2	1.73911758401344\\
2.25	1.60258353063648\\
2.35	1.34721263134395\\
2.4	1.22978583469682\\
2.5	1.01456609863752\\
2.55	0.915874912948097\\
2.65	0.735269509940908\\
2.7	0.653034732628049\\
2.8	0.503142301164947\\
2.9	0.372868019094847\\
2.95	0.314699765128569\\
3.05	0.212678524974066\\
3.15	0.128003204897181\\
3.25	0.0581245777579669\\
3.35	0.00182276357666341\\
3.45	0.0472707583930905\\
3.55	0.0834238884700527\\
3.65	0.108808587498543\\
3.75	0.12514467847989\\
3.9	0.13594896671684\\
4	0.136085502503457\\
4.1	0.131474255075421\\
4.25	0.11720342284128\\
4.35	0.103132538979509\\
4.5	0.0769064144203751\\
4.65	0.0490310237342113\\
4.75	0.0310826247264486\\
4.9	0.00716651816400384\\
5.05	0.0114874401516752\\
5.2	0.0253097143903967\\
5.4	0.0361744724609941\\
5.55	0.0332919458788617\\
5.7	0.0358568746268852\\
5.9	0.0302696028182518\\
6.05	0.0200453218897189\\
6.25	0.0108146827641572\\
6.45	0.00198107515059182\\
6.65	0.00554341408557572\\
6.85	0.0113024388184722\\
7.05	0.0147269747329646\\
7.25	0.0155205118607727\\
7.45	0.0141429647699469\\
7.7	0.00560885189499022\\
7.95	0.00437990560427451\\
8.15	0.000775903493263964\\
8.4	0.00648012074628341\\
8.65	0.0036072888891211\\
8.95	0.00301208630736289\\
9.2	0.00556550493285136\\
9.5	0.00294387966306969\\
9.75	0.00332557013814198\\
10.05	0.00507547805703217\\
10.35	0.00563739013591374\\
10.7	0.000400831212214498\\
11	0.00129318902617594\\
11.35	0.00130985328907412\\
11.7	0.00358980412727658\\
12.05	0.000834259779924434\\
};
\addlegendentry{$q=3$}

\addplot [color=mycolor1, dashed]
  table[row sep=crcr]{%
1	7\\
15	0.0311111111111111\\
};
\addlegendentry{$R^{-2}$}

\addplot [color=mycolor2, dashed]
  table[row sep=crcr]{%
1	60\\
15	0.00118518518518519\\
};
\addlegendentry{$R^{-4}$}

\end{axis}
\end{tikzpicture}%
